Simulation Intelligence: Towards a New Generation of Scientific Methods

The original "Seven Motifs" set forth a roadmap of essential methods for the field of scientific computing, where a motif is an algorithmic method that captures a pattern of computation and data movement. We present the "Nine Motifs of Simulation Intelligence", a roadmap for the development and integration of the essential algorithms necessary for a merger of scientific computing, scientific simulation, and artificial intelligence. We call this merger simulation intelligence (SI), for short. We argue the motifs of simulation intelligence are interconnected and interdependent, much like the components within the layers of an operating system. Using this metaphor, we explore the nature of each layer of the simulation intelligence operating system stack (SI-stack) and the motifs therein: (1) Multi-physics and multi-scale modeling; (2) Surrogate modeling and emulation; (3) Simulation-based inference; (4) Causal modeling and inference; (5) Agent-based modeling; (6) Probabilistic programming; (7) Differentiable programming; (8) Open-ended optimization; (9) Machine programming. We believe coordinated efforts between motifs offers immense opportunity to accelerate scientific discovery, from solving inverse problems in synthetic biology and climate science, to directing nuclear energy experiments and predicting emergent behavior in socioeconomic settings. We elaborate on each layer of the SI-stack, detailing the state-of-art methods, presenting examples to highlight challenges and opportunities, and advocating for specific ways to advance the motifs and the synergies from their combinations. Advancing and integrating these technologies can enable a robust and efficient hypothesis-simulation-analysis type of scientific method, which we introduce with several use-cases for human-machine teaming and automated science.

==> mp.tex <==
% !TeX root = ./main.tex

\subsection*{9. MACHINE PROGRAMMING}

\textit{Machine programming (MP)} is the automation of software (and potentially hardware) development.  Machine programming is a general technology, in ways that are quite different than the other simulation intelligence motifs. As systems based on the simulation intelligence motifs grow in complexity, at some point these systems will necessitate automating aspects of software development. Machine programming can understand code across motifs, compose them into working systems, and then optimize these systems to execute on the underlying hardware -- this interaction is illustrated in Fig. \ref{fig:os} at a high-level. Hence, while MP is not tied to any specific class of SI problems, MP will be integral as the glue that ties the other motifs together, serving as a bridge to the hardware. 

The term \emph{Machine Programming} made its debut in a paper by Gottschlich et al.~\cite{gottschlich:2018:mapl} that defined the MP in terms of three distinct pillars: \emph{(i)} \emph{intention}, \emph{(ii)} \emph{invention}, and \emph{(iii)} \emph{adaptation} (Fig. \ref{fig:pillars}). \emph{Intention} is principally concerned with identifying novel ways and simplifying existing ways for users to express their ideas to a machine. It is also concerned with lifting meaning (i.e., semantics) from existing software and hardware systems~\cite{ahmad:2019:siggraph, kamil:2016:pldi, lee:2021:plp}. \emph{Invention} aims to construct the higher-order algorithms and data structures that are necessary to fulfill a user's intention. In many cases, inventive systems simply fuse existing components together to form a novel solution that fulfills the user's intent. However, there are some corner cases, which are likely to become more prevalent in the future, where an inventive system constructs a truly novel solution  not yet been discovered by humans (e.g., Alam et al.'s inventive performance regression testing system~\cite{alam:2019:neurips} and Li and Malik's inventive optimization algorithm system~\cite{li:2017:iclr}). \emph{Adaptation} takes an \emph{invented} high-order program and adapts it to a specific hardware and software system. This is done to ensure certain quality characteristics are maintained such as correctness, performance, security, maintainability, and so forth.

If trends continue, we anticipate programming languages will become more intentional by design. The byproduct of such intentionality is that such languages will be capable of more holistic automation of the inventive and adaptive pillars of MP, while simultaneously achieving super-human levels in key quality characteristics (e.g., software performance, security, etc.). Early evidence has emerged demonstrating this such as Halide~\cite{adams:2019:siggraph}, a domain-specific programming language embedded in C++, which has been designed for high-performance image and array processing code on modern hardware (various CPU and GPU architectures) and operating systems (Linux, Android, etc.). Halide, in conjunction with verified lifting, has demonstrably improved the performance of Adobe Photoshop by a geometric mean of $3.36x$ for approximately 300 transpiled functions~\cite{ahmad:2019:siggraph}. Moreover, other forms of intentional communication from humans to machines are already emerging, such as translation from natural language to software programs, and also from visual diagrams to software program translation. Two embodiments of such systems are GitHub's Co-Pilot~\cite{Chen2021EvaluatingLL} and Ellis et al.'s automated synthesis of code for visual diagrams~\cite{ellis:2018:neurips}.


\begin{figure}[htpb]
\begin{center}
\includegraphics[width=0.5\columnwidth]{figures/three_pillars.pdf}
% \vspace{-0.2cm}
\caption{The ``Three Pillars of Machine Programming'': intention, invention, adaptation.
Intention is quite literally to discover the intent of the programmer, and to lift meaning from software. Example sub-domains include program synthesis and inductive programming, which share territory with the Invention pillar, for creating new algorithms and data structures. Sketch~\cite{nye:2019:infer}, FlashFill~\cite{Gulwani2011AutomatingSP}, and DeepCoder~\cite{Balog2017DeepCoderLT} are notable examples, with many others noted in text and in \cite{gottschlich:2018:mapl}.
The adaptation pillar is for evolving in a changing hardware/software world, and more broadly in dynamic systems of data, sensors, and people \cite{lavin2021technology} -- examples include X and Y?
(Figure reproduced from Gottschlich et al.~\cite{gottschlich:2018:mapl})
}
\label{fig:pillars}
\end{center}
\end{figure}

% \subsubsection*{The Bifurcated Space of Machine Programming}

\begin{figure}[htpb!]
\begin{center}
\includegraphics[width=0.9\columnwidth]{figures/bifurcated-space-mp.png}
% \vspace{-0.2cm}
\caption{The ``Bifurcated Space of Machine Programming''.}
\label{fig:mpbifurcation}
\end{center}
\end{figure}

In machine programming, there appear to be at least two fundamental approaches for automation. The first is \emph{stochastic}, which consist of things such as machine learning and statistical analysis~\cite{alam:2019:neurips, hasabnis:2021:maps}. The second is \emph{deterministic}, which consist of approaches using formal methods that might include techniques such as satisfiability solvers (SAT solvers) or satisfiability modulo theory (SMT) solvers~\cite{alur:2013:fm, kamil:2016:pldi}.

As the field of MP matures, we are already seeing an emergence of systems that consist of both stochastic and deterministic elements. A concrete example of this is Solar-Lezama et al.'s work fusing formal sketching techniques (where a \textit{program sketch} is the schematic outline of a full program) with deep neural networks to improve computational tractability~\cite{nye:2019:infer}. Another example is the Machine Inferred Code Similarity (MISIM) system by Ye et al., which uses a deterministic context-aware semantics structure (CASS) in conjunction with a learned similarity scoring system driven by a Siamese deep neural network~\cite{ye:2020:misim}. 

%\paragraph{The Importance of Data for MP}
%
%- explain 'data' areas of the 3 pillars figure
%
%- ControlFlag, labeled data repos (POJ-104, Google Code Jam, IBM/MIT Project CodeNet, Microsoft's CodeXGlue)
%

% \paragraph{MP and simulation sciences}

%
%
% \subsection*{Examples}\label{sec:MP_ex}
%
% In this section we provide a small number of concrete MP systems, both as research systems and production-quality industrial systems. We segment the space based on the three pillars of MP to facilitate an easier understanding of our belief of the systems' main contributions.

%\paragraph{Intention --}
%Perhaps the most important pillar to separate from the others is that of \emph{intention}. The reason for this is such separation generally enables the inventive and adaptive MP systems to function more exhaustively in their reasoning about the possible solution space of the user's provided intent when it does not contain artificial bindings to invention and adaptation. Two examples of such intentional MP systems are Halide~\cite{jrk:2013:pldi} and verified lifting~\cite{kamil:2016:pldi}.

%We consider Halide to be one of the most intentional programming languages in existence today, because of its separation of concerns design. Invented by Jonathan Ragan-Kelley, Halide is designed to be programmed by two different types of programmers for any given program: the \emph{algorithmic} programmer and the \emph{scheduling} programmer. In this context the algorithmic programmer is the user providing the intention of what should be done (i.e., the image processing details to apply to an image). The scheduling programmer provides the optimized computational steps to most effectively execute the image processing details specified by the algorithmic programmer. However, while Halide was initially designed for two types of programmers, the scheduling programmer has most recently been replaced by an MP inventive and adaptive system as described by Adams et al.~\cite{adams:2019:siggraph}.

%\paragraph{Invention}
%
%- Define program synthesis (here?)
%
%- Ryan Marcus's Neo query optimization system, AutoPerf, Learning to Optimize
%
%\paragraph{Adaptation}
%
%- Saman's stuff: TACO, Tiaramasu, GraphIT, Ryan's Bao

% \paragraph{The Importance of Data for MP}

% - ControlFlag, labeled data repos (POJ-104, Google Code Jam, IBM/MIT Project CodeNet, Microsoft's CodeXGlue)


\subsection*{Future directions}\label{sec:MP_future}

One of the core directions the field of MP is heading is towards \emph{intentional programming}. Intentional programming is principally concerned with separating the intention of the program from the components that are used to realize that intention. A critical reason for this \emph{separation of concerns} is that it tends to enable the machine to handle more of the inventive and adaptive components of software development. A concrete embodiment of this is seen in the Halide programming language, where the Halide auto-scheduler can write more performant software (in the form of code, not neural networks) than the best humans it was pit against, which includes those individuals who developed the language itself~\cite{adams:2019:siggraph}.

We anticipate the field of MP to help accelerate the development and deployment of the SI stack. Referring back to the SI operating system conceptualization in Fig. \ref{fig:os}, without MP one can imagine bottom-up constraints on the types of data structures and algorithms that can be implemented above the hardware layers
This is not unlike a ``hardware lottery'', where a research idea or technology succeeds and trumps others because it is suited to the available software and hardware, not necessarily because it is superior to alternative directions \cite{Hooker2021TheHL}.
Historically this has been decisive in the paths pursued by the largely disconnected hardware, systems, and algorithms communities; the past decade provides an industry-shaping example with the marriage of deep learning and GPUs. The various mechanisms of MP, however, provide opportunity to mitigate such hardware lottery effects for SI, and broadly in the AI and software fields. With MP in the SI operating system, as a motif that interfaces hardware and software, the integration of SI motifs can become far more efficient (auto HW-SW optimizations and codesign), robust (less prone to human and stochastic errors), and scalable (flexibly deployable modules from HPC to the edge).
% The same abstraction can be drawn to science and engineering broadly, where a research idea wins because it is suited to the available software and hardware and not because the idea is superior to alternative research directions.




